GastroVision: A Multi-class Endoscopy Image Dataset for Computer Aided Gastrointestinal Disease Detection

Integrating real-time artificial intelligence (AI) systems in clinical practices faces challenges such as scalability and acceptance. These challenges include data availability, biased outcomes, data quality, lack of transparency, and underperformance on unseen datasets from different distributions. The scarcity of large-scale, precisely labeled, and diverse datasets are the major challenge for clinical integration. This scarcity is also due to the legal restrictions and extensive manual efforts required for accurate annotations from clinicians. To address these challenges, we present \textit{GastroVision}, a multi-center open-access gastrointestinal (GI) endoscopy dataset that includes different anatomical landmarks, pathological abnormalities, polyp removal cases and normal findings (a total of 27 classes) from the GI tract. The dataset comprises 8,000 images acquired from B{\ae}rum Hospital in Norway and Karolinska University Hospital in Sweden and was annotated and verified by experienced GI endoscopists. Furthermore, we validate the significance of our dataset with extensive benchmarking based on the popular deep learning based baseline models. We believe our dataset can facilitate the development of AI-based algorithms for GI disease detection and classification. Our dataset is available at \url{https://osf.io/84e7f/}.

==> takeout.tex <==

% Dataset details links
% CVC-VideoClinicDB: https://giana.grand-challenge.org/PolypDetection/
% CVC-ClinicDB, ETIS-Larib, Asu-Mayo: https://polyp.grand-challenge.org/Databases/, http://refbase.cvc.uab.es/files/BSV2011e.pdf
% Kvasir-SEG: https://datasets.simula.no/kvasir-seg/
% SUN Database: http://sundatabase.org/
% PolypSet: https://dataverse.harvard.edu/dataset.xhtml?persistentId=doi:10.7910/DVN/FCBUOR
%Kvasir-Capsule: https://osf.io/dv2ag/
%KID: https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5452962/pdf/10-1055-s-0043-105488.pdf
%\vspace{-5mm}


%from Olympus (Olympus Europe,
%Germany) and Pentax (Pentax Medical Europe, Germany)
%The four hospitals associated with VV provide healthcare services to around 490,000 people and among these hospitals, Bærum Hospital alone serves 189,000 people. 
% Annotation done by ????
% Consent ???
%\subsection{Positive samples}
%\subsection{Negative samples}
%\subsubsection{Annotation strategies and quality assurance}


%The macro precision, recall, and F1-score are obtained by calculating the average of the class-wise F1-scores. Similarly, macro recall and macro precision are computed. The micro F1-score is calculated as the harmonic mean of macro-averaged precision and macro-averaged recall. The micro recall and micro precision consider class-wise true positives with class-wise false negatives and false positives, respectively.  %To compute these metrics for a multi-class classification problem like ours, micro and macro averages are considered for each of the three metrics.

%\begin{figure} [t]
%    \centering
%    \includegraphics[width=0.9\linewidth]{Figures/gast_result.png}
%    \caption{Graph depicting the class-wise performance associated with the best outcome obtained using pre-trained DenseNet-121.}
%    \label{fig:result_graph}
%\end{figure}


%, there is evidence that with each 1.0\% increase in adenoma detection rate (ADR), there is an associated 3.0% decrease in the risk of interval CRC.9 10 However,
%polyps can be missed, with reported miss rates of
%up to 27% due to both polyp and operator charac-teristics


\textbf{{It is estimated that about 11.3\% of upper GI neoplasms and 2.1\%-5.9\% polyps in lower GI are overlooked during EGD and colonoscopy, respectively~\cite{turshudzhyan2022lessons}}}.

%It also includes shape and stage (advanced/ non-advanced) annotations of lesions.

%\item The dataset can be used to train, validate, and compare the performance of existing and future AI models on a comprehensive set of GI finding classes. This can aid in developing state-of-the-art solutions and computer-aided systems for GI disease detection. 


%Apart from SUN Database, the \textbf{PolypsSet}~\cite{li2021colonoscopy,patel2020comparative} dataset also provides pathological annotations with bounding box annotations, except that it contains only binary classification labels, i.e., adenomatous and hyperplastic. It consists of 28,773 frames in the training set, 4,254 frames for validation, and 4,872 frames for testing that belong to 116, 17, and 22 video sequences, respectively.


%\par \textbf{Challenges:} 
%These procedures involve acquiring videos from inside the GI tracts using high-definition endoscopes and, thus, demand resources such as expensive equipment and trained clinicians. Further, 

 %\textbf{inflammatory lesions}, \textbf{melanosis} (darkening of the colon lining), and \textbf{scars}. 
%The examination accuracy also depends on the image quality and can be hampered by some artifacts. Such cases involve images with \textbf{bubble artifacts}, \textbf{dirty colon feces}, \textbf{seeds}, and surgical \textbf{tools}. Therapeutic interventions are required to treat the detected lesion. These lesions are marked for a follow-up or surgery using a medical technique called \textbf{tattooing}.

%PolypsSet~\cite{li2021colonoscopy,patel2020comparative} & Polyps & 37,899 image frames$^\clubsuit$ & Public\\ \hline

%Colon diverticula refer to small, pouch-like protrusions that can develop along the colon's wall, particularly in areas where the natural muscular layers of the colon are weaker. The normal mucosa and vascular pattern in the large bowel play a pivotal role in maintaining digestive function and overall health. Colorectal cancer is a malignant growth that originates in the colon or rectum. The terminal ileum is the final segment of the small intestine, connecting to the large intestine. The normal colon, a vital component of the lower gastrointestinal tract, performs essential functions in digestion, absorption, and elimination. 




%, and is expected to complement the performance of AI-based techniques. 
%The dataset can further be used to compare existing and future models in computer vision and the medical domain.

%In this paper, we present a new multi-class endoscopy dataset, $GastroVision$, for GI anomaly and disease detection. It is released as an open-access resource for the research community and is expected to complement the performance of AI-based techniques. Together with the dataset we also release the source code for the experiments. The image data and corresponding annotations could allow researchers to formulate methodologies not only for classifying different anatomical and pathological findings but also for further categorizing lesions according to shape and stage (advanced/non-advanced). We evaluated the dataset using some baseline models and standard multi-class classification metrics. The results show that XXX some insight that call for future work XXX. The dataset can further be used to compare existing and future models in computer vision and the medical domain. Having a diverse set of categories labeled by expert endoscopists, $GatroVision$ is unique and valuable for computer-aided GI anomaly and disease detection, patient examinations, and medical training.         
% 
% \subsubsection*{Acknowledgement}
% This project is partially supported by the NIH funding: R01-CA246704 and R01-CA240639.


% \section*{Accessibility}
% Authors are kindly asked to make their submissions as accessible as possible for everyone including people with disabilities and sensory or neurological differences.
% Tips of how to achieve this and what to pay attention to will be provided on the conference website \url{http://icml.cc/}.

% \section*{Software and Data}
% If a paper is accepted, we strongly encourage the publication of software and data with the  % camera-ready version of the paper whenever appropriate. This can be % done by including a URL in the camera-ready copy. However, \textbf{do not} % include URLs that reveal your institution or identity in your % submission for review. Instead, provide an anonymous URL or upload % the material as ``Supplementary Material'' into the CMT reviewing  system. Note that reviewers are not required to look at this material % when writing their review.


 \textbf{Gastric polyps} are abnormal growths in the stomach lining. \textbf{Ulcers} are the open sores in the stomach or duodenum that can lead to discomfort and bleeding. \textbf{Esophageal varices} result from portal hypertension, causing swollen veins in the esophagus. \textbf{Erythema} refers to redness, often indicating inflammation and \textbf{blood in the lumen} denotes bleeding. \textbf{Accessory tools} aid in investigating and diagnosing upper and lower GI tract conditions for targeted treatment.


  \textbf{Gastric polyps} are abnormal growths in the stomach lining. \textbf{Ulcers} are the open sores in the stomach or duodenum that can lead to discomfort and bleeding. \textbf{Esophageal varices} result from portal hypertension, causing swollen veins in the esophagus. \textbf{Erythema} refers to redness, often indicating inflammation and \textbf{blood in the lumen} denotes bleeding. \textbf{Accessory tools} aid in investigating and diagnosing upper and lower GI tract conditions for targeted treatment.
